BertGCN: Transductive Text Classification by Combining GCN and BERT

In this work, we propose BertGCN, a model that combines large scale pretraining and transductive learning for text classification. BertGCN constructs a heterogeneous graph over the dataset and represents documents as nodes using BERT representations. By jointly training the BERT and GCN modules within BertGCN, the proposed model is able to leverage the advantages of both worlds: large-scale pretraining which takes the advantage of the massive amount of raw data and transductive learning which jointly learns representations for both training data and unlabeled test data by propagating label influence through graph convolution. Experiments show that BertGCN achieves SOTA performances on a wide range of text classification datasets. Code is available at https://github.com/ZeroRin/BertGCN.

==> ablation.tex <==
\subsection{The Effect of $\lambda$}
\begin{figure}
    \centering
    \includegraphics[scale=0.65]{20ng_m.png}%
    \caption{Text accuracy of RoBERTaGCN when varying $\lambda$ on 20NG. The dotted line indicates the corresponding RoBERTa baseline.}
    \label{fig:lambda}
\end{figure}

$\lambda$ controls the trade-off between training BertGCN and BERT. The optimal value of $\lambda$ can be different for different tasks. Fig.\ref{fig:lambda} shows the accuracy of RoBERTaGCN with different $\lambda$. On 20NG, the  accuracy is consistently higher with larger $\lambda$ value. This can be explained by the high performance of graph-based methods on 20NG. 
The model reaches its best when $\lambda=0.7$, performing slightly better than only using the GCN prediction ($\lambda=1$). 
%On R8 where BERT methods have better performance, a balanced prediction may be needed. 



\subsection{The Effect of Strategies in Joint Training }
\begin{table}
  \small
  \centering
  \scalebox{0.85}{
  \begin{tabular}{lcccc}\toprule
    {\bf Strategy} & {\it w/ both} & {\it w/o finetune} & {\it w/o small lr.} & {\it w/o both}\\
    {\bf Accuracy} & 89.5 & 88.0 & 9.0 & 8.8\\
    \bottomrule
  \end{tabular}}
  \caption{Results on 20NG for different strategies. ``finetune'' means we use the finetuned RoBERTa as initialization, and ``small lr.'' means we use a smaller learning rate for the RoBERTa module.}
  \label{tab:ab_init_lr}
\end{table}

To overcome inconsistency of embeddings in the memory bank, we set a smaller learning rate for the BERT module and use a finetuned BERT model for initialization. We evaluate the effect of the two strategies. Table \ref{tab:ab_init_lr} shows the  results of RoBERTaGCN on 20NG with and without these strategies. 
With the same learning rate for RoBERTa and GCN, the model cannot be trained due to inconsistency in the memory bank, regardless of whether the fine-tuned RoBERTa is used. Models can be successfully trained when we set a smaller learning rate for the RoBERTa module, and additional using finetuned RoBERTa leads to the best performance.


==> experiments.tex <==
\section{Experiments}
\subsection{Datasets and Baselines}
We run experiments on five widely-used  text classification benchmarks: 20 Newsgroups (20NG)\footnote{\url{http://qwone.com/˜jason/20Newsgroups/}}, R8 and R52\footnote{\url{https://www.cs.umb.edu/~smimarog/textmining/datasets/}}, Ohsumed\footnote{\url{http://disi.unitn.it/moschitti/corpora.htm}} and Movie Review (MR) \citep{pang-lee-2005-seeing}\footnote{\url{http://www.cs.cornell.edu/people/pabo/movie-review-data/}}. 

We compare BertGCN to current state-of-the-art pretrained and GCN models: TextGCN \citep{yao2019graph}, SGC \citep{wu2019simplifying}, BERT \citep{devlin2018bert} and RoBERTa \citep{yinhan2019roberta}. Details for datasets and baseline are left in the supplementary material.

\subsection{Settings}

We follow protocols in textGCN \citep{yao2019graph} to preprocess data. 
For BERT and RoBERTa, we use the output feature of the [CLS] token as the document embedding, followed by a feedforward layer to derive the final prediction. We use BERT$_\text{base}$ and a two-layer GCN to implement BertGCN. We initialize the learning rate to 1e-3 for the GCN module and 1e-5 for the fine-tuned BERT module. We also implement RoBERTaGCN that uses RoBERTa instead of BERT. 

\subsection{Main Results}

\begin{table}
  \small
  \centering
  \scalebox{0.9}{
  \begin{tabular}{lccccc}\toprule
    {\bf Model} & {\bf 20NG} & {\bf R8} & {\bf R52} & {\bf Ohsumed} & {\bf MR}\\
    \midrule 
    {\it TextGCN}  &  86.3& 97.1& 93.6& 68.4 &76.7\\
    {\it SGC} & 88.5 &97.2 &94.0 & 68.5 & 75.9\\
%    {\it SSGC} & 88.6 &97.4& 94.5 & 68.5 & 76.7\\
    \cdashline{1-6}
    {\it BERT} & 85.3 & 97.8 & 96.4 & 70.5 & 85.7\\
    {\it RoBERTa} & 83.8 & 97.8 & 96.2 & 70.7 & 89.4\\
    \cdashline{1-6}
    {\it BertGCN} & 89.3  & 98.1 & \bf{96.6} & \bf{72.8} & 86.0 \\
    % test under the same lambda as corresponding RoBERTaGCN
    {\it RoBERTaGCN} & {\bf 89.5} & {\bf 98.2} & 96.1 & {\bf 72.8} & {\bf 89.7}\\
    \bottomrule
  \end{tabular}
  }
  \caption{Results for different models on transductive text classification datasets. We run all models 10 times and report the mean test accuracy.}
  \label{tab:main}
\end{table}


Table \ref{tab:main} presents the test accuracy of each model. We can see that BertGCN and RoBERTaGCN perform the best across all datasets. Only using BERT and RoBERTa generally performs better than  GCN variants except 20NG, which is due to the great merits brought by large-scale pretraining. 
Compared with BERT and RoBERTa, the performance boost from BertGCN and RoBERTaGCN
 is significant on the 20NG and Ohsumed datasets. This is because the average length in 20NG and Ohsumed is much longer than that in other datasets:
the graph is constructed using word-document statistics, which means that long texts may produce more document connections transited via an intermediate word node, and this potentially benefits message passing through the graph, leading to better performances when combined with GCN.
% \begin{itemize}
%     \item The graph is constructed using word-document statistics, which means that long texts may produce more document connections transited via an intermediate word node. This potentially benefits message passing through the graph.
%     \item BERT-based models may suffer from long texts, as it is harder for the model to ``pay attention to'' the key components of the document when there are many words.
% \end{itemize}
This may also explain why GCN models perform better than BERT models on 20NG.
For datasets with shorter documents such as R52 and MR, the power of graph structure is limited, and thus the performance boost is smaller relative to 20NG. 
%Nevertheless, since we introduced a strategy that balances the prediction of both models, the performance of BertGCN are consistently better than the corresponding RoBERTa performance. 

==> method.tex <==
\section{Method}
%In this section, we first introduce how our BertGCN model combine BERT and GCN model together for text classification, then we explain how to jointly train both parts of the model in a end-to-end manner.

\subsection{BertGCN}

%TextGCN \citep{yao2019graph} proves that text graph is a powerful tool in text classification problem. However, it uses identity matrix for node features, which completely ignores the document contents. We suggest that the content of the documents should be equally important. 
In the proposed BertGCN model, 
we initialize  representations for document nodes in a text graph 
using
 a BERT-style model (e.g., BERT, RoBERTa).
 These representations 
   are used as inputs to GCN. 
 Document  representations will then be iteratively updated based on the graph structures  using GCN, the outputs of which are treated as final representations for document nodes, 
 and are sent to the softmax classifier for predictions. 
In this way,
 we are able to  leverage the complementary strengths of pretrained models and graph models.

% In the proposed BertGCN model, we first finetune a BERT \citep{devlin2018bert} or RoBERTa \citep{yinhan2019roberta} model on specific datasets. Then we use the finetuned model to extract document embeddings, which are used as initialization for the corresponding document nodes in the GCN model. This makes it possible to fully leverage the complementary strengths of the pretrained model and the graph model.

Specifically, we construct a heterogeneous graph containing both word nodes and document nodes following TextGCN \citep{yao2019graph}. We define word-document edges and word-word edges based on the term frequency-inverse document frequency (TF-IDF) and positive point-wise mutual information (PPMI), respectively. The weight of an edge between two nodes $i$ and $j$ is defined as:  {\color{red} equation}
\begin{align*}
\footnotesize
    \begin{split}
    A_{i,j}= \left \{
        \begin{array}{ll}
            \operatorname{PPMI}(i, j), & i, j\text{ are words and } i \neq j \\
            \operatorname{TF-IDF}(i, j),     & i\text{ is document, }j\text{ is word}\\
            1, & i = j\\
            0, & \text{otherwise}
        \end{array}
    \right.
    \end{split}
\end{align*}
In TextGCN, an identity matrix is used as initial node features $X = I_{n_\text{doc}+n_\text{word}}$, where $n_\text{doc}$ is the number of document nodes, $n_\text{word}$ is the number of word nodes (including both training and test), and $I$ denotes the identify matrix. 
In BertGCN, we use a BERT-style model  to obtain the  document embeddings, and treat them as input representations for document nodes. 
%The document embeddings contain information about document semantics, which is crucial for classification tasks. 
 Document node embeddings are denoted by $X_\text{doc}\in\mathbb{R}^{n_\text{doc}\times d}$, where $d$ is the embedding dimensionality.
%We initialize word node embeddings as all-zero vectors.\footnote{} 
Overall, the initial node feature matrix is given by:
 $$
 X= \left (
        \begin{array}{c}
            X_\text{doc}\\
            0
        \end{array}
 \right )_{(n_\text{doc}+n_\text{word})\times d}
 $$


\begin{comment}
The document node features are computed as
$$
F_{doc} = f_\theta(X)
$$
where $X$ indicates the matrix of input token sequences for documents, and $f$ is a BERT model with parameters $\theta$ that encodes token sequences to embedding vectors. $F_{doc}$ is a $n_{doc} \times d$ matrix where $n_{doc}$ is the number of document nodes and $d$ is the dimension of the document embedding.
\end{comment}
 
We feed $X$ into a GCN model \citep{kipf2016semi}. GCN iteratively propagates messages across training and test examples. Specifically {\color{red} GCN fomular}. 

Outputs from GCN are treated as final representations for documents.  Representations for documents in the training dataset are fed to the softmax layer for classification:
\begin{equation}
Z_\text{GCN} = \operatorname{softmax}(g(X, A))
\label{gcn}
\end{equation}

where $g$ is the GCN model. 
We use the cross entropy loss over labeled document nodes to jointly optimize parameters for BERT and GCN.
%$$ \mathcal{L} = -\sum_{d\in \mathcal{Y}_D}\sum_{c=0}^{C-1} Y_{d,c} \operatorname{ln} Z_{d,c}$$
%where $\mathcal{Y}_D$ is the set of document indices with training labels, $C$ is the number of classes and $Y$ is the one-hot label matrix.
 
 \subsection{Balancing BERT and GCN Predictions}
%The text graph provide explicit links among related documents, which helps make better prediction. However, the complex structure of text graph can be confusing, and make it harder for optimization. Moreover, it is possible for the model to be misleading. On the other hand, make prediction directly based on the extracted document embeddings will not have these concerns, while it loses the chance to benefit from the graph structure.
Practically, we find that jointly training BERT and GCN in a multi-task setup leads to faster convergence and better performances. 
For BERT training, we follow the vanilla BERT, where the [CLS] representations (denoted by $X$) are fed to the softmax layer: 
\begin{equation}
  Z_\text{BERT} = \operatorname{softmax}(WX)
\end{equation}

The final training objective is the 
linear interpolation of the prediction from BertGCN and the prediction from BERT, which is given by:
\begin{align*}
    Z &= \lambda Z_\text{GCN} + (1-\lambda) Z_\text{BERT}
\end{align*} 
where $\lambda$ controls the tradeoff between the two objectives. 
$\lambda=1$ means we use the full BertGCN model, and $\lambda=0$ means we only use the BERT module. When $\lambda\in (0,1)$, we are able to balance the predictions from both models, and the BertGCN model can be better optimized.

The explanation for better performances achieved by the multi-task interpolation is as follows: $X$ are used as inputs to the multi-layer structure of GCN. The  multi-layer  structure of GCN
suffers from intrinsic drawbacks such as gradient vanishing or over-smoothing {\color{red} citation}. 
The $Z_\text{BERT}$ directly operates on the input to the   multi-layer GCN structure (i.e., $X$), which 
  makes sure that  inputs to GCN are regulated and optimized towards the  objective, and thus  leads to better performances. 



 \subsection{Optimization using Memory Bank}
 
%The original GCN model uses full-batch gradient descent method for training, which requires to store intermediate embeddings for all nodes. The memory requirement of such method grows linerly as the number of node grows. Since GCN models are usually shallow and do not contain many parameters, this only becomes trouble when the number of node is extremely large. In our BertGCN model, however, this effect is problematic even with small graph, since it indicates that we need to do full batch training for both BERT and GCN model, which is impractical with limited resource. \citep{hamilton2017inductive} proposed neighbor sampling to enable mini-batch training on GCN, but this is still not satisfactory for BertGCN. If we sample $d$ neighbors at each layer, for a GCN with $l$ layer, the effective batch-size will be $1/d^l$ of the possible batch-size for BERT model. The maxium batch-size for BERT model limits the size of input node set for GCN, which then limits the batch-size of GCN.

The original GCN model uses the full-batch gradient descent method for training, which is intractable for the proposed BertGCN model, since the full-batch method can not be applied to BERT due to the memory limitation.
Inspired by techniques in contrastive learning which decouples the dictionary size from the mini-batch size \citep{wu2018unsupervised,he2020momentum}, we introduce a memory bank that stores all document embeddings to decouple the training batch size from the total number of nodes in the graph.
 
Specifically, during training, we maintain a memory bank $M$ that tracks input features for all document nodes. At the beginning of each epoch, we first compute all document embeddings using the {\it current} BERT module and store them in $M$. During each iteration, we sample a mini batch from both labeled and unlabeled document nodes with the index set $I = \{i_0, i_1...i_b\}$, where $b$ is the mini-batch size. We then compute their document embeddings $M_I$ also using the {\it current} BERT module and update the corresponding memories in $M$.\footnote{Note that the BERT module used to compute $M_I$ is the one finished training in the last iteration, which is different from the the BERT module used to compute the initial $M$.}
Next, we use the updated $M$ as input to derive the GCN output and compute the loss for the current mini batch. For back-propagation, $M$ is considered as constant except the records in $I$.

With the memory bank, we are able to efficiently train the BertGCN model including the BERT module.
However, during training, the embeddings in the memory bank are computed using the BERT module at different steps in an epoch and are thus inconsistent. To overcome this issue, we set a small learning rate for the BERT module to improve consistency of the stored embeddings. With low learning rate the training takes more time. In order to speed up training, we fine-tune a BERT model on the target dataset before training begins, and use it to {\bf initialize} the BERT parameters  in  BertGCN.
